PreSTU: Pre-Training for Scene-Text Understanding

The ability to recognize and reason about text embedded in visual inputs is often lacking in vision-and-language (V&L) models, perhaps because V&L pre-training methods have often failed to include such an ability in their training objective. In this paper, we propose PreSTU, a novel pre-training recipe dedicated to scene-text understanding (STU). PreSTU introduces OCR-aware pre-training objectives that encourage the model to recognize text from an image and connect it to the rest of the image content. We implement PreSTU using a simple transformer-based encoder-decoder architecture, combined with large-scale image-text datasets with scene text obtained from an off-the-shelf OCR system. We empirically demonstrate the effectiveness of this pre-training approach on eight visual question answering and four image captioning benchmarks.

==> discuss.tex <==
%auto-ignore
\section{Considerations and Limitations}
\label{sec:discuss}
We use mT5~\cite{mt5} designed for multilingual tasks as our language model but only experiment on English scene-text \vl datasets in this paper. We will further evaluate our \ourmodel on multilingual scene-text \vl tasks like EST-VQA~\cite{wang2020general}.

Due to time and resource constraints, we conduct our experiments with a relatively small \vl model (160M parameters) compared to existing works (\eg, GIT and Flamingo have 0.8B and 80B parameters, respectively). In future work, we will scale up our model to further validate \ourmodel's effectiveness on scene-text \vl tasks.




==> reviewer_comment.tex <==
%auto-ignore
\newcommand{\Rone}{{\color{purple} R1}}
\newcommand{\Rtwo}{{\color{teal} R2}}
\newcommand{\Rthree}{{\color{blue} R3}}
\newcommand{\myparatop}[1]{\vspace{0mm}\noindent\textbf{#1}.}

\section{Reviewer Comment}
\mypar{\Rone}
\begin{itemize} [itemsep=0pt,topsep=0.1pt,leftmargin=10pt]
    \item As paper mentioned, ocr texts are ordered based on their locations, top-left to bottom-right. It would be valueable if the model can utilize the coordinates of the text bboxes since it would provide explicit location information for pre-training text reading module.
    \item I would like to see a bit more analysis on general encoder-decoder designs other than mT5.
    \item PreSTU seems a general architecture, thus except for STVQA task, can it be applied to other domains, e.g., docVQA?
    %\item Final review: The rebuttal does not entirely address my concerns (e.g., use of location features, architectural designs.). The authors do not provide experimental results to support their clarification.
\end{itemize}

\mypar{\Rtwo}
\begin{itemize} [itemsep=0pt,topsep=0.1pt,leftmargin=10pt]
    \item The paper does not compare with correct prior-art in STVQA and TextVQA. LaTr is a CVPR 2022 Oral paper and it significantly outperforms PreSTU on at least two datasets. ST-VQA (LaTr: 69.6 vs PreSTU: 65.5), gap of 4.1 anls. on Text-VQA (LaTr: 61.60, TextVQA: 55.2), gap of 6.4 anls.
    \item Table 3 and 4 shows that the w/wo PreSTU training the performance improves across all tasks. However the more important knowledge addition to the community is to know if this methodology of training is better than prior art on those datasets. Here things are not clear. Proposed approach PreSTU does not beat prior-art (GIT and Flamingo. also please note LaTr should have been compared here). This could be because of smaller PreSTU model of less pre-training data. Not knowing this likely to cause confusion to an independent researcher.
    \item Authors claim they start from mT5 which has been pre-trained on vast amounts of data. It is unclear how much performance gains are coming purely from starting off with mT5 weights vs the proposed pre-training tasks and fine-tuning. Zero-shot mT5 on proposed datasets is missing.
    \item In Sec 3.1 some of the advantages stated using T5 based enc-dec models give robustness of OCR, the model being vocabulary-free have been proposed and explored in LaTr (CVPR 2022 Oral), however it has not been cited. Please note the benefits of using multi-modal based enc-dec model for text-VQA has been explored in LaTr preceding the work done by GIT and Flamingo. The authors of this paper do not compare (in experimental section) or give appropriate citation through-out the paper for LaTr e.g., Sec. 3.1 (lines 297-310), Sec 3.2 (lines 389-392)
    \item mT5 is bigger in number of parameters than T5 (used by LaTr), can the authors please provide the parameter count of their approach?
    \item LaTr uses 224x224 image resolution whereas PreSTU uses 640x640 which likely given it an advantage. Apples to apples comparison is needed to gauge the real impact of this paper.
    \item It is unclear how the method handles scenarios where there is no scene-text in the image (either due to OCR error or the image does not have any scene-text). Is PreSTU performance robust to this scenario?
    \item L106, I do not agree to this statement - premise is faulty? “the image context is not fully represented, in spite of it being often relevant to understanding” how are the authors making this claim? LaTr and TAP uses image features and also object detection networks.
    \item Line 117 feels like a misplaced citation. [48] does not make sense here. Citing TAP would make more sense as it uses pre-detected objects.
    \item Line 134, which off-the-shelf OCR system? As the quality of OCR has big impact on the performance.
    %\item Final review: I thank the authors for their rebuttal. However, I maintain my rating of Weak Reject owing to my concerns not entirely addressed in the rebuttal and also based on the observations from peer reviewers.
\end{itemize}

\mypar{\Rthree}
\begin{itemize} [itemsep=0pt,topsep=0.1pt,leftmargin=10pt]
    \item Although I understand that the main contribution relates to the pre-training strategy, the employed architecture is a combination of existing components (i.e. ViT and mT5) thus limiting the technical novelty from an architectural point of view.
    \item My most important concern is related to the lack of an important scene-text VQA competitor (i.e. LaTr [6]) in the experimental comparison. In particular, it is not clear why the authors decided not to compare their model with this recently proposed approach, especially since it is one of the few papers proposing pre-training strategies in the context of scene-text VQA. Moreover, LaTr [6] seems to perform better than the model proposed in this paper on some considered benchmarks.
    \item From the results, it is not clear whether the improvement over previous methods such as TAP [62] is due to the proposed pre-training strategy or to the more powerful vision/language backbones. In my opinion, it would have been interesting to see the results of the proposed PreSTU model using the pre-training objectives of TAP or, instead, by re-training TAP with at least the same visual backbone (finetuned during training) used in this paper.
    \item Following GIT [58] and LaTr[6], the results on the OCR-VQA dataset [45] are missing.
    \item It would have been interesting to see the results of a variant of the SPLITOCR pre-training objective with random masking of some OCR tokens, thus recalling the typical masked language modeling objective.
    %\item Final review: The authors' response does not entirely address my main concerns regarding the lack of relevant experimental comparisons with existing methods. After reading other reviews, I think the paper is slightly below the acceptance threshold of a top-tier conference like CVPR.
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%% Our Response %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\noindent We thank all the reviewers. They find our idea ``novel and intuitive'' (\Rone), and ``interesting'' (\Rthree); our paper ``well-written and easy to follow'' (\Rone, \Rthree), and ``well-organized'' (\Rone); our results ``interesting'' (\Rtwo), and ``shown in both quantitatively and qualitatively'' (\Rone, \Rthree). We address the major comments below and will incorporate all feedback (\Rone: iWEv, \Rtwo: YuXQ, \Rthree: 51KM).

\myparatop{Other scene-text domains (\Rone, \Rthree)}
During rebuttal, we evaluate PreSTU on 4 other VQA \& 2 other captioning tasks (\autoref{tab:other_domains_reb}); in total, 12 tasks. PreSTU is also effective on book, document, illustration, and screenshot domains.

\myparatop{Comparison to LaTr and prior arts (\Rtwo, \Rthree)}
We promise to give proper credits to LaTr in Sect.~3.1. We initially include methods that work on both image captioning \& VQA (LaTr does not consider image captioning). 
Following your suggestion, we will include LaTr results in our comparison.
We reiterate that the main goal of our experiments is to show the utility of our pre-training objectives (L460-462). All reviewers agree this is well-supported by our results on 6 benchmarks (+6 in this rebuttal). For context, LaTr only focuses on 2 \emph{VQA} tasks; TAP on 3.

While both PreSTU and LaTr focus on pre-training for STU using an encoder-decoder architecture, there are \textbf{conceptual differences}.
First, LaTr focuses on pre-training on document images. Their claim is that this is a better choice since acquiring large quantities of natural images with scene text for pre-training is challenging and hard to scale and the amount of text is often sparse.
Our work challenges this assumption and shows that \emph{one can pre-train effectively for STU on natural images with minimal preprocessing.}
Second, LaTr's pre-training objective achieves a different goal and does \textbf{not} involve a ``visual component'' during pre-training; it focuses on modeling the co-occurrence stats of layout-aware OCR tokens.
In contrast, we aim to learn both scene-text recognition and the role of scene text in its ``visual context'' (L124-126). What we learn leads to strong results on our downstream tasks \emph{even without} OCR signals as input (Table 5, L640-732).
We believe this message is \textbf{valuable} and \textbf{complementary} to LaTr's. It even suggests a research direction of designing an effective pre-training strategy that works with both types of data.

Quantitatively, we first want to point out that it becomes harder to use ``digits'' to compare methods due to the large discrepancy in the settings and the high cost of performing apples-to-apples comparison.
Noticing this difficulty, we do not claim state-of-the-art results throughout the paper, even when our approach outperforms GIT/Flamingo (L529-533), which consider much larger models and data. Note that we explicitly mention architectures, model and data sizes as context in Table 3 and 4.
More specific to LaTr, apples-to-apples comparison has to consider factors beyond image resolution and is difficult due to (i) no official code release, (ii) partially available data (OCR-IDL), and (iii) discrepancy between OCR systems.
Our base model is weaker; NoPreSTU achieves 45.2\% on TextVQA, while LaTr-Base with no pre-training achieves strong 52.29\% (better than TAP, a strong baseline \emph{with pre-training}).
With pre-training, PreSTU achieves a large gain (10.4\%) wrt LaTr's gain (3.99\%).
With similar model/data sizes, PreSTU/13M is only slightly behind LaTR-base/11M (55.6\% vs. 56.28\%).

\begin{table}[t]
\centering
% \small
\footnotesize
\tabcolsep 1pt
%\renewcommand\arraystretch{1.0}
\vspace{-5mm}
\begin{tabular}{ccccccc}
\toprule
\multirow{3}{*}{Model} & OCR & Doc & Chart & \multirow{2}{*}{AI2D} & Widget & Screen2 \\
& VQA & VQA & QA & & Cap & Words \\
 & \%Acc & \%ANLS & \%RelaxedAcc & \%Acc & CIDEr & CIDEr  \\
\midrule
NoPreSTU & 71.5 & 47.5 & 40.5 & 64.5 & 63.9 & 98.5 \\
\midrule
PreSTU-SplitOCR & 72.2 & 50.1 & 50.7 & 69.3 & 125.6 & 113.8\\
\bottomrule
\end{tabular}
\vspace{-2mm}
\captionsetup{width=.85\textwidth} 
\caption{\small \textbf{PreSTU on other scene-text domains (val split)}}
\label{tab:other_domains_reb}
\vspace{-7mm}
\end{table}

\myparatop{Coordinates of OCR texts (\Rone)} We can include an analysis of this in the final version (due to limited rebuttal time).

\myparatop{Encoder-decoder design (\Rone)} mT5 is based on a general transformer-based encoder-decoder architecture. Thus, we believe our insights can be applied to other encoder-decoder models (\eg, BART). We will include more analysis.

\myparatop{mT5's zero-shot performance (\Rtwo)}
mT5 is trained on span corruption, quite far from our downstream tasks. It achieves low zero-shot performance of 0.04\% (Table 6). This gets improved to 56.7\% with our pre-training scheme, justifying the effectiveness of our approach.

\myparatop{Parameter count (\Rtwo)}
LaTr uses T5-base/large (172/722M); PreSTU mT5-base (192M). The extra parameters of mT5-base vs.~T5-base are in the 1st layer to cover a larger vocab of multilingual tokens, which do not bring advantages to the English-only benchmarks we consider.

\myparatop{Non-scene-text scenarios (\Rtwo)} Without detected scene text, our model relies on the image to make predictions. Thus, our approach achieves robust performance on general VQAv2, where most images have no scene text (L489-498).

\myparatop{L106 (\Rtwo)} The claim refers to TAP which only uses FRCNN detection features, based on Visual Genome's 1600 objects/400 attributes. We thus believe image pixels provide a less lossy context. We will make this point clearer.

\myparatop{Off-the-shelf OCR (\Rtwo)} Google Cloud OCR (L323-324).

\myparatop{Novelty (\Rthree)}
\Rthree{} correctly points out that our main contribution is the pre-training strategy, and we deliberately choose a general model architecture to push for its applicability.
We believe that such a design choice, along with the notable gains, makes our results more convincing and should not be seen as a weakness.

\myparatop{Improvement by objectives or backbones (\Rthree)} 
We note that a strict apples-to-apples comparison is ideal but hard to achieve, as pre-training objectives are often coupled with model architectures (\eg, TAP relies on detected objects and their features, but PreSTU does not.) Yet, we try to make a fair comparison in L538-570; we compare Non-TAP and NoPreSTU, both without pre-training. They achieve similar performance on TextVQA \& TextCaps, suggesting that they have similar backbone quality. With OCR-specific pre-training, however, PreSTU notably outperforms TAP.


\mypar{Should we include PaLI or not?}

\mypar{if include:}

\mypar{Pros}
\begin{itemize} [itemsep=0pt,topsep=0.1pt,leftmargin=10pt]
    \item Applicability of PreSTU. PaLI used our \ourocr to learn scene-text recognition and achieved SOTA.
    \item PaLI already mentioned PreSTU. ``Following Kil et al. (2022), we order the OCR items based on their locations...'', ``OCR on WebLI OCR-text data ... (Kil et al., 2022)''
    \item Avoid the same complaint. If we don't compare to PaLI, future reviewers may complain again: why we did not compare to PaLI which is SOTA.
\end{itemize}
\mypar{Cons}
\begin{itemize} [itemsep=0pt,topsep=0.1pt,leftmargin=10pt]
    \item Perhaps, more follow-up experiments needed. Reviewers may ask: why don't we take PaLI as our base model and do analysis of our objectives -->
    But, here I'm not sure if reviewers ask these experiments because: Our PreSTU was released first (arXiv) than PaLI, and PaLI already mentioned that they used our objective to learn scene-text recognition during pre-training. So, not sure if these experiments are necessary... (kind of reversing experiments in terms of the release timeline) 
\end{itemize} 
--------------------------------------------------------------------
\mypar{Checklist}
\begin{itemize} [itemsep=0pt,topsep=0.1pt,leftmargin=10pt]
    \item Moved Related Work to the end for the better paper structure: With the current structure, hard to go back and forth between the paragraph and the corresponding Table.
    \item Removed Qualtiative Results (Figure 4) to save the space: We may remove Figure 4 since we already have Figure 1.
    \item All co-author registers?
\end{itemize}
